RAN Slicing Performance Trade-offs: Timing versus Throughput Requirements

The coexistence of diverse services with heterogeneous requirements is a fundamental feature of 5G. This necessitates efficient radio access network (RAN) slicing, defined as sharing of the wireless resources among diverse services while guaranteeing their respective throughput, timing, and/or reliability requirements. In this paper, we investigate RAN slicing for an uplink scenario in the form of multiple access schemes for two user types: (1) broadband users with throughput requirements and (2) intermittently active users with timing requirements, expressed as either latency-reliability (LR) or Peak Age of Information (PAoI). Broadband users transmit data continuously, hence, are allocated non-overlapping parts of the spectrum. We evaluate the trade-offs between the achievable throughput of a broadband user and the timing requirements of an intermittent user under Orthogonal Multiple Access (OMA) and Non-Orthogonal Multiple Access (NOMA), considering capture. Our analysis shows that NOMA, in combination with packet-level coding, is a superior strategy in most cases for both LR and PAoI, achieving a similar LR with only slight 2% decrease in throughput with respect to the upper bound in performance. However, there are extreme cases where OMA achieves a slightly greater throughput than NOMA at the expense of an increased PAoI.

==> figs/access.tex <==
\begin{tikzpicture}[>=latex]
% fill with packets


\foreach \i in {1,2,3,5,6,7}
    \draw[fill=white!70!blue,draw=none] (\i,4) rectangle (\i+1,3);
\foreach \i in {4,8}
    \draw[fill=white!70!yellow,draw=none] (\i,4) rectangle (\i+1,3);
\foreach \i in {1,...,8}
    \draw[fill=white!70!green,draw=none] (\i,2) rectangle (\i+1,1);
% \foreach \i in {5,6}
%     \draw[fill=white!70!green,draw=none] (\i,0) rectangle (\i+1,-1);
% \foreach \i in {1,2,3,4,7,8}
%     \draw[fill=white!70!blue,draw=none] (\i,0) rectangle (\i+1,-1);
    
% \foreach \i in {1,...,8}
%     \draw[] (\i,0cm) -- ++(1cm,0) -- ++(0,-1cm) -- ++(-1cm,0) -- ++ (0,1cm);
\foreach \i in {1,...,8}
    \draw[] (\i,2cm) -- ++(1cm,0) -- ++(0,-1cm) -- ++(-1cm,0) -- ++ (0,1cm);
\foreach \i in {1,...,8}
    \draw[] (\i,4cm) -- ++(1cm,0) -- ++(0,-1cm) -- ++(-1cm,0) -- ++ (0,1cm);
    
% \node at (1.5,-1.3) {\large $1$};
% \node at (2.5,-1.3) {\large $2$};
% \node at (3.5,-1.3) {\large $3$};
% \node at (4.5,-1.3) {\large $4$};
% \node at (5.5,-1.3) {\large $N\!-\!1$};
% \node at (6.5,-1.3) {\large $N$};
% \node at (7.5,-1.3) {\large $1$};
% \node at (8.5,-1.3) {\large $2$};

\node at (1.5,0.7) {\large $1$};
\node at (2.5,0.7) {\large $2$};
\node at (3.5,0.7) {\large $3$};
\node at (4.5,0.7) {\large $4$};
\node at (5.5,0.7) {\large $N\!-\!1$};
\node at (6.5,0.7) {\large $N$};
\node at (7.5,0.7) {\large $1$};
\node at (8.5,0.7) {\large $2$};

\node at (1.5,2.7) {\large $1$};
\node at (2.5,2.7) {\large $2$};
\node at (3.5,2.7) {\large $3$};
\node at (5.5,2.7) {\large $4$};
\node at (6.5,2.7) {\large $N\!-\!1$};
\node at (7.5,2.7) {\large $N$};

    
\node [anchor=east] (OMA) at (1,3.5) {\large OMA};
\node [below=2cm of OMA.east,anchor=east] {\large NOMA};
% \node [below=4cm of OMA.east,anchor=east] {\large PNOMA};
\node at (10,3.5) {\huge $\cdots$};
\node at (10,1.5) {\huge $\cdots$};
% \node at (10,-0.5) {\huge $\cdots$};
    

\draw[fill=white!70!blue] (11.2cm,4cm) -- ++(0.5cm,0) -- ++(0,-0.5cm) -- ++(-0.5cm,0) -- ++ (0,0.5cm);
\node[anchor=west] (BB) at (11.8cm,3.7cm) {\large Broadband};
\draw[fill=white!70!yellow] (11.2cm,3cm) --  ++(0.5cm,0) -- ++(0,-0.5cm) -- ++(-0.5cm,0) -- ++ (0,0.5cm);
\node [below=1cm of BB.west,anchor=west] {\large Intermittent};
\draw[fill=white!70!green] (11.2cm,2cm) -- ++(0.5cm,0) -- ++(0,-0.5cm) -- ++(-0.5cm,0) -- ++ (0,0.5cm);
\node [below=2cm of BB.west,anchor=west] {\large Mixed};

\draw (10.7,4.5) rectangle (14.4,1);

\draw[-{Latex[length=3mm]}] (1,4.8) -- node[midway,above] {\large Time} (10,4.8);
\draw[{|[scale=2.0]}-{|[scale=2.0]}] (4,4.4) -- node[midway,fill=white] {\large $T_\text{int}$} (8,4.4);
\draw[{|[scale=2.0]}-{|[scale=2.0]}] (1,0.2) -- node[midway,below] {\large Slot} (2,0.2);
\draw[{|[scale=2.0]}-{|[scale=2.0]}] (1,-0.4) -- node[midway,below] {\large Frame} (7,-0.4);


% 
% \draw [fill=white!90!green,draw=none] (2,-1) rectangle (1.6,0); 
% \draw [fill=white!90!green,draw=none] (1.6,-1) rectangle (1.2,0); 
% \draw [fill=white!90!green,draw=none] (1.2,-1) rectangle (0.8,0); 
% \draw [fill=white!90!blue,draw=none] (2,1) rectangle (1.6,2); 
% \draw [fill=white!90!blue,draw=none] (1.6,1) rectangle (1.2,2); 
% \draw [fill=white!90!red,draw=none] (2,-2) rectangle (1.6,-3); 
% 
% \draw [fill=white!90!green,draw=none] (6,-1) rectangle (5.6,0);
% \draw [fill=white!90!red,draw=none] (5.6,-1) rectangle (5.2,0);
% \draw [fill=white!90!red,draw=none] (5.2,-1) rectangle (4.8,0);
% \draw [fill=white!90!blue,draw=none] (4.8,-1) rectangle (4.4,0);
% 
% 
% \draw [fill=white!90!green,draw=none] (10,-1) rectangle (9.6,0); 
% \draw [fill=white!90!blue,draw=none] (10,1) rectangle (9.6,2); 
% \draw [fill=white!90!blue,draw=none] (9.6,1) rectangle (9.2,2); 
% \draw [fill=white!90!blue,draw=none] (9.2,1) rectangle (8.8,2); 
% \draw [fill=white!90!red,draw=none] (10,-2) rectangle (9.6,-3); 
% \draw [fill=white!90!red,draw=none] (9.6,-2) rectangle (9.2,-3); 
% 
% 
% % the rectangle with vertical rules
% \draw[green] (0,0) -- ++(2cm,0) -- ++(0,-1cm) -- ++(-2cm,0);
% \draw[blue] (0,2) -- ++(2cm,0) -- ++(0,-1cm) -- ++(-2cm,0);
% \draw[red] (0,-2) -- ++(2cm,0) -- ++(0,-1cm) -- ++(-2cm,0);
% 
% 
% \foreach \i in {1,...,4}
%   \draw[green] (2cm-\i*0.4cm,0) -- +(0,-1cm);
% \foreach \i in {1,...,4}
%   \draw[blue] (2cm-\i*0.4cm,2) -- +(0,-1cm);
% \foreach \i in {1,...,4}
%   \draw[red] (2cm-\i*0.4cm,-2) -- +(0,-1cm);
%   
%   
% \draw (4cm,0) -- ++(2cm,0) -- ++(0,-1cm) -- ++(-2cm,0);
% \foreach \i in {1,...,4}
%   \draw (6cm-\i*0.4cm,0) -- +(0,-1cm);
% 
% 
% \draw[blue] (8cm,2) -- ++(2cm,0) -- ++(0,-1cm) -- ++(-2cm,0);
% \draw[red] (8cm,-2) -- ++(2cm,0) -- ++(0,-1cm) -- ++(-2cm,0);
% \draw[green] (8cm,0) -- ++(2cm,0) -- ++(0,-1cm) -- ++(-2cm,0);
% \foreach \i in {1,...,4}
%   \draw[green] (10cm-\i*0.4cm,0) -- +(0,-1cm);
% \foreach \i in {1,...,4}
%   \draw[red] (10cm-\i*0.4cm,-2) -- +(0,-1cm);
% \foreach \i in {1,...,4}
%   \draw[blue] (10cm-\i*0.4cm,2) -- +(0,-1cm);
% 
% 
% 
% % the circle
% \draw[green] (2.5,-0.5cm) circle [radius=0.5cm];
% \draw (6.5,-0.5cm) circle [radius=0.5cm];
% \draw[green] (10.5,-0.5cm) circle [radius=0.5cm];
% 
% \draw[red] (2.5,-2.5cm) circle [radius=0.5cm];
% \draw[blue] (2.5,1.5cm) circle [radius=0.5cm];
% \draw[blue] (10.5,1.5cm) circle [radius=0.5cm];
% \draw[red] (10.5,-2.5cm) circle [radius=0.5cm];
% 
% % the arrows and labels
% \draw[<-,green] (4,-0.5) -- +(-1,0);
% \draw[<-,blue] (4,-0.5) -- +(-1,2);
% \draw[<-,red] (4,-0.5) -- +(-1,-2);
% \draw[->,green] (7,-0.5) -- +(1,0);
% \draw[->,blue] (7,-0.5) -- +(1,2);
% \draw[->,red] (7,-0.5) -- +(1,-2);
% \draw[->,green] (11,-0.5) -- +(1,0);
% \draw[->,blue] (11,1.5) -- +(1,0);
% \draw[->,red] (11,-2.5) -- +(1,0);
% 
% \draw[<-,green] (0,-0.5) -- +(-20pt,0) node[left] {$\lambda$};
% \draw[<-,red] (0,-2.5) -- +(-20pt,0) node[left] {$\lambda$};
% \draw[<-,blue] (0,1.5) -- +(-20pt,0) node[left] {$\lambda$};
% \node at (6.5,-0.5) {ISL};
% \node at (2.5,-0.5) {\textcolor{green}{ISL}};
% \node at (10.5,-0.5) {\textcolor{green}{DL}};
% \node at (2.5,-2.5) {\textcolor{red}{ISL}};
% \node at (10.5,-2.5) {\textcolor{red}{DL}};
% \node at (2.5,1.5) {\textcolor{blue}{ISL}};
% \node at (10.5,1.5) {\textcolor{blue}{DL}};
\end{tikzpicture}


==> figs/access_bwp.tex <==

    
\begin{tikzpicture}[>=latex]
% fill with packets
\pgfmathsetmacro{\yfob}{-2.8}
\pgfmathsetmacro{\yfoi}{-1.3}
\pgfmathsetmacro{\yoma}{2.5}
\pgfmathsetmacro{\ynoma}{1}


\foreach \i in {1,2,...,8}
    {\draw[fill=Set3-B,draw=black] (\i,\yfoi+1) rectangle (\i+1,\yfoi);
    \draw[fill=Blues-G,draw=black] (\i,\yfob+1) rectangle (\i+1,\yfob);}
    

\foreach \i in {1,2,3,5,6,7}
    \draw[fill=Blues-G,draw=black] (\i,\yoma+1) rectangle (\i+1,\yoma);
\foreach \i in {4,8}
    \draw[fill=Set3-B,draw=black] (\i,\yoma+1) rectangle (\i+1,\yoma);
\foreach \i in {1,...,8}{
    \draw[fill=Blues-G,draw=black] (\i,\ynoma+1) rectangle (\i+1,\ynoma);
    \draw[pattern=custom north west lines,hatchspread=4pt,hatchthickness=1pt,hatchcolor=Set3-B](\i,\ynoma+1) rectangle (\i+1,\ynoma);
    }
    

% \foreach \i in {5,6}
%     \draw[fill=color2,draw=none] (\i,0) rectangle (\i+1,-1);
% \foreach \i in {1,2,3,4,7,8}
%     \draw[fill=Blues-G,draw=none] (\i,0) rectangle (\i+1,-1);
    
% \foreach \i in {1,...,8}
%     \draw[] (\i,0cm) -- ++(1cm,0) -- ++(0,-1cm) -- ++(-1cm,0) -- ++ (0,1cm);

    
% \node at (1.5,-1.3) {\large $1$};
% \node at (2.5,-1.3) {\large $2$};
% \node at (3.5,-1.3) {\large $3$};
% \node at (4.5,-1.3) {\large $4$};
% \node at (5.5,-1.3) {\large $N\!-\!1$};
% \node at (6.5,-1.3) {\large $N$};
% \node at (7.5,-1.3) {\large $1$};
% \node at (8.5,-1.3) {\large $2$};

\node[fill=Blues-G, inner sep=1, circle] at (1.5,\ynoma+0.5) {\large $1$};
\node[fill=Blues-G, inner sep=1, circle] at (2.5,\ynoma+0.5) {\large $2$};
\node[fill=Blues-G, inner sep=1, circle] at (3.5,\ynoma+0.5) {\large $3$};
\node[fill=Blues-G, inner sep=1, circle] at (4.5,\ynoma+0.5) {\large $4$};
\node[fill=Blues-G, inner sep=1, circle] at (5.5,\ynoma+0.5) {\large $5$};
\node[fill=Blues-G, inner sep=1, circle] at (6.5,\ynoma+0.5) {\large $N$};
\node[fill=Blues-G, inner sep=1, circle] at (7.5,\ynoma+0.5) {\large $1$};
\node[fill=Blues-G, inner sep=1, circle] at (8.5,\ynoma+0.5) {\large $2$};

\node at (1.5,\yoma+0.5) {\large $1$};
\node at (2.5,\yoma+0.5) {\large $2$};
\node at (3.5,\yoma+0.5) {\large $3$};
\node at (5.5,\yoma+0.5) {\large $4$};
\node at (6.5,\yoma+0.5) {\large $5$};
\node at (7.5,\yoma+0.5) {\large $N$};

\node at (1.5,\yfob+0.5) {\large $1$};
\node at (2.5,\yfob+0.5) {\large $2$};
\node at (3.5,\yfob+0.5) {\large $3$};
\node at (4.5,\yfob+0.5) {\large $4$};
\node at (5.5,\yfob+0.5) {\large $5$};
\node at (6.5,\yfob+0.5) {\large $N$};
\node at (7.5,\yfob+0.5) {\large $1$};
\node at (8.5,\yfob+0.5) {\large $2$};


    
\node [anchor=east] (OMA) at (1,\yoma+0.5) {\large TDMA};
\node [anchor=east] at (1,\ynoma+0.5){\large NOMA};

%\node [anchor=east] at (1,\yfoi-0.125){\large FOS};
\draw [decorate,decoration={brace,amplitude=5pt,raise=4pt},yshift=0pt]
(1,\yfob) -- (1, \yfoi+1) node [black,midway, anchor=east, xshift=-8pt, align=center] {\large FDMA\\(benchmark)};

% \node [below=4cm of OMA.east,anchor=east] {\large PNOMA};
\node at (10,\yoma+0.5) {\huge $\cdots$};
\node at (10,\ynoma+0.5) {\huge $\cdots$};
\node at (10,\yfoi+0.5) {\huge $\cdots$};
\node at (10,\yfob+0.5) {\huge $\cdots$};
% \node at (10,-0.5) {\huge $\cdots$};
    
\begin{scope}[yshift=-1cm]
\draw[fill=Blues-G] (11.2cm,4cm) -- ++(0.5cm,0) -- ++(0,-0.5cm) -- ++(-0.5cm,0) -- ++ (0,0.5cm);
\node[anchor=west] (BB) at (11.8cm,3.7cm) {\large Broadband};
\draw[fill=Set3-B] (11.2cm,3cm) --  ++(0.5cm,0) -- ++(0,-0.5cm) -- ++(-0.5cm,0) -- ++ (0,0.5cm);
\node [below=1cm of BB.west,anchor=west] {\large Intermittent};

\draw[fill=Blues-G] (11.2cm,2cm) -- ++(0.5cm,0) -- ++(0,-0.5cm) -- ++(-0.5cm,0) -- ++ (0,0.5cm);
\draw[pattern=custom north west lines,hatchspread=4pt,hatchthickness=1pt,hatchcolor=Set3-B] (11.2,2) rectangle (11.7,1.5);
\node [below=2cm of BB.west,anchor=west] {\large Mixed};

\draw (10.7,4.5) rectangle (14.4,1);
\end{scope}

\draw[-{Latex[length=3mm]}] (1,\yoma+2.2) --++ (10,0)node[midway,above] {\large Time};
\draw[{|[scale=2.0]}-{|[scale=2.0]}] (4,\yoma+1.4) --++ (4,0)node[midway,fill=white] {\large $T_\text{int}$};
\draw[{|[scale=2.0]}-{|[scale=2.0]}] (1,\yoma+1.4) --++  (1,0)node[midway,above] {\large Slot};
\draw[{|[scale=2.0]}-{|[scale=2.0]}] (1,\ynoma-0.4) --++ (6,0)node[midway,below] {\large Frame};

\end{tikzpicture}


==> figs/optimal_config/throughput_fdma.tex <==
\begin{tikzpicture}
\begin{axis}[
width=\fwidth,
height=\fheight,
axis lines*=box,
xlabel={Coded block size $N$},
legend cell align={left},
legend style={ at={(0.98,0.07)}, anchor=south east, font=\footnotesize,
fill opacity=0.75,
text opacity=1,
draw opacity=1,
  draw=white!80!black,
},
xmajorgrids,
ymajorgrids,
tick align=outside,
tick pos=left,
xmin=0,
xmax=32,
ymin=0,
ymax=1,
xtick distance=4,
]
\addplot[YlGnBu-J, semithick] table [x index=0, y index=2] {figs/optimal_config/optimal_KforN.txt};
\addplot[Set2-B, semithick] table [x index=0, y index=3] {figs/optimal_config/optimal_KforN.txt};
\addplot[Dark2-A, semithick] table [x index=0, y index=4] {figs/optimal_config/optimal_KforN.txt};
\legend{Maximum throughput $S$, Success probability $p_{s,1}$, Optimal coding ratio $K/N$} 
\end{axis}
\end{tikzpicture}

==> figs/simple_access.tex <==
\begin{tikzpicture}[>=latex]
% fill with packets


    

\foreach \i in {1,2,3,5,6,7}
    \draw[fill=white!70!blue,draw=none] (\i,6) rectangle (\i+1,4);
\foreach \i in {4,8}
    \draw[fill=white!70!yellow,draw=none] (\i,6) rectangle (\i+1,4);
\draw[fill=white!70!yellow,draw=none] (1,3) rectangle (9,4);
\foreach \i in {1,...,8}
    \draw[fill=white!70!green,draw=none] (\i,2) rectangle (\i+1,-1);
    
\foreach \i in {1,...,8}
    \draw[] (\i,0cm) -- ++(1cm,0) -- ++(0,-1cm) -- ++(-1cm,0) -- ++ (0,1cm);
\foreach \i in {1,...,8}
    \draw[] (\i,1cm) -- ++(1cm,0) -- ++(0,-1cm) -- ++(-1cm,0) -- ++ (0,1cm);
\foreach \i in {1,...,8}
    \draw[] (\i,2cm) -- ++(1cm,0) -- ++(0,-1cm) -- ++(-1cm,0) -- ++ (0,1cm);
\foreach \i in {1,...,8}
    \draw[] (\i,4cm) -- ++(1cm,0) -- ++(0,-1cm) -- ++(-1cm,0) -- ++ (0,1cm);
\foreach \i in {1,...,8}
    \draw[] (\i,5cm) -- ++(1cm,0) -- ++(0,-1cm) -- ++(-1cm,0) -- ++ (0,1cm);
\foreach \i in {1,...,8}
    \draw[] (\i,6cm) -- ++(1cm,0) -- ++(0,-1cm) -- ++(-1cm,0) -- ++ (0,1cm);
    
\node [anchor=east] (OMA) at (1,4.5) {\large OMA};
\node [below=4cm of OMA.east,anchor=east] {\large NOMA};
\node at (10,2.5) {\huge $\cdots$};
\node at (10,4.5) {\huge $\cdots$};


\draw[fill=white!70!blue] (11.2cm,4cm) -- ++(0.5cm,0) -- ++(0,-0.5cm) -- ++(-0.5cm,0) -- ++ (0,0.5cm);
\node[anchor=west] (BB) at (11.8cm,3.7cm) {\large Service 1};
\draw[fill=white!70!yellow] (11.2cm,3cm) --  ++(0.5cm,0) -- ++(0,-0.5cm) -- ++(-0.5cm,0) -- ++ (0,0.5cm);
\node [below=1cm of BB.west,anchor=west] {\large Service 2};
\draw[fill=white!70!green] (11.2cm,2cm) -- ++(0.5cm,0) -- ++(0,-0.5cm) -- ++(-0.5cm,0) -- ++ (0,0.5cm);
\node [below=2cm of BB.west,anchor=west] {\large Mixed};

\draw (10.7,4.5) rectangle (14.4,1);

\draw[-{Latex[length=3mm]}] (-1,6.8) -- node[midway,above] {\large Time} (10,6.8);
\draw[-{Latex[length=3mm]}] (-1,6.8) -- node[midway,left] {\large Frequency} (-1,-2);
\draw[{|[scale=2.0]}-{|[scale=2.0]}] (4,6.4) -- node[midway,fill=white] {\large $T_\text{int}$} (8,6.4);
\draw[{|[scale=2.0]}-{|[scale=2.0]}] (8,-1.8) -- node[midway,below] {\large Timeslot} (9,-1.8);
\draw[{|[scale=2.0]}-{|[scale=2.0]}] (9.8,0) -- node[midway,right] {\large Subchannel} (9.8,-1);


\end{tikzpicture}

